Interference Suppression Using Deep Learning: Current Approaches and Open Challenges

In light of the finite nature of the wireless spectrum and the increasing demand for spectrum use arising from recent technological breakthroughs in wireless communication, the problem of interference continues to persist. Despite recent advancements in resolving interference issues, interference still presents a difficult challenge to effective usage of the spectrum. This is partly due to the rise in the use of license-free and managed shared bands for Wi-Fi, long term evolution (LTE) unlicensed (LTE-U), LTE licensed assisted access (LAA), 5G NR, and other opportunistic spectrum access solutions. As a result of this, the need for efficient spectrum usage schemes that are robust against interference has never been more important. In the past, most solutions to interference have addressed the problem by using avoidance techniques as well as non-AI mitigation approaches (for example, adaptive filters). The key downside to non-AI techniques is the need for domain expertise in the extraction or exploitation of signal features such as cyclostationarity, bandwidth and modulation of the interfering signals. More recently, researchers have successfully explored AI/ML enabled physical (PHY) layer techniques, especially deep learning which reduces or compensates for the interfering signal instead of simply avoiding it. The underlying idea of ML based approaches is to learn the interference or the interference characteristics from the data, thereby sidelining the need for domain expertise in suppressing the interference. In this paper, we review a wide range of techniques that have used deep learning to suppress interference. We provide comparison and guidelines for many different types of deep learning techniques in interference suppression. In addition, we highlight challenges and potential future research directions for the successful adoption of deep learning in interference suppression.

==> ref.tex <==
@inproceedings{qiu2007general,
  title={A general model of wireless interference},
  author={Qiu, Lili and Zhang, Yin and Wang, Feng and Han, Mi Kyung and Mahajan, Ratul},
  booktitle={Proceedings of the 13th annual ACM international conference on Mobile computing and networking},
  pages={171--182},
  year={2007}
}

@article{bruno2007interference,
  title={Interference Reduction in Wireless Networks},
  author={Bruno, Joseph},
  journal={Computing Research Topics, Computing Sciences Department, Villanova University},
  year={2007}
}

@incollection{laster1995survey,
  title={A Survey of adaptive single channel interference rejection techniques for wireless communications},
  author={Laster, JD and Reed, JH},
  booktitle={Wireless Personal Communications},
  pages={29--53},
  year={1995},
  publisher={Springer}
}

@article{carrick2019mitigating,
  title={Mitigating linear-frequency-modulated pulsed radar interference to {OFDM}},
  author={Carrick, Matt and Reed, Jeffrey H and Spooner, Chad M},
  journal={IEEE Transactions on Aerospace and Electronic Systems},
  volume={55},
  number={3},
  pages={1146--1159},
  year={2019},
  publisher={IEEE}
}

@inproceedings{balatsoukas2018non,
  title={Non-linear digital self-interference cancellation for in-band full-duplex radios using neural networks},
  author={Balatsoukas-Stimming, Alexios},
  booktitle={2018 IEEE 19th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@inproceedings{jain2011practical,
  title={Practical, real-time, full duplex wireless},
  author={Jain, Mayank and Choi, Jung Il and Kim, Taemin and Bharadia, Dinesh and Seth, Siddharth and Srinivasan, Kannan and Levis, Philip and Katti, Sachin and Sinha, Prasun},
  booktitle={Proceedings of the 17th annual international conference on Mobile computing and networking},
  pages={301--312},
  year={2011}
}

@inproceedings{bharadia2013full,
  title={Full duplex radios},
  author={Bharadia, Dinesh and McMilin, Emily and Katti, Sachin},
  booktitle={Proceedings of the ACM SIGCOMM 2013 conference on SIGCOMM},
  pages={375--386},
  year={2013}
}

@inproceedings{shi2019digital,
  title={Digital self-interference cancellation for full duplex wireless communication based on neural networks},
  author={Shi, Chengzhe and Hao, Yuefan and Liu, Ying and Shao, Shihai},
  booktitle={2019 4th International Conference on Communication and Information Systems (ICCIS)},
  pages={53--57},
  year={2019},
  organization={IEEE}
}

@article{korpi2017nonlinear,
  title={Nonlinear self-interference cancellation in {MIMO} full-duplex transceivers under crosstalk},
  author={Korpi, Dani and Anttila, Lauri and Valkama, Mikko},
  journal={EURASIP journal on wireless Communications and Networking},
  volume={2017},
  number={1},
  pages={1--15},
  year={2017},
  publisher={Springer}
}

@inproceedings{anttila2014modeling,
  title={Modeling and efficient cancellation of nonlinear self-interference in {MIMO} full-duplex transceivers},
  author={Anttila, Lauri and Korpi, Dani and Antonio-Rodr{\'\i}guez, Emilio and Wichman, Risto and Valkama, Mikko},
  booktitle={2014 IEEE Globecom Workshops (GC Wkshps)},
  pages={777--783},
  year={2014},
  organization={IEEE}
}

@inproceedings{islam2019comprehensive,
  title={A comprehensive self-interference model for single-antenna full-duplex communication systems},
  author={Islam, Md Atiqul and Smida, Besma},
  booktitle={ICC 2019-2019 IEEE International Conference on Communications (ICC)},
  pages={1--7},
  year={2019},
  organization={IEEE}
}

@article{muranov2021deep,
  title={On Deep Learning Assisted Self-Interference Estimation in a Full-Duplex Relay Link},
  author={Muranov, Konstantin and Islam, Md Atiqul and Smida, Besma and Devroye, Natasha},
  journal={IEEE Wireless Communications Letters},
  year={2021},
  publisher={IEEE}
}

@inproceedings{kurzo2018design,
  title={Design and implementation of a neural network aided self-interference cancellation scheme for full-duplex radios},
  author={Kurzo, Yann and Burg, Andreas and Balatsoukas-Stimming, Alexios},
  booktitle={2018 52nd Asilomar Conference on Signals, Systems, and Computers},
  pages={589--593},
  year={2018},
  organization={IEEE}
}

@inproceedings{guo2019dsic,
  title={{DSIC}: Deep learning based self-interference cancellation for in-band full duplex wireless},
  author={Guo, Hanqing and Wu, Shaoen and Wang, Honggang and Daneshmand, Mahmoud},
  booktitle={2019 IEEE Global Communications Conference (GLOBECOM)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@inproceedings{yang2010iterative,
  title={Iterative narrowband interference suppression for ds-cdma systems using feed-forward neural network},
  author={Yang, Zan and Zhao, Tingting and Zhao, Yuping and Yu, Jianli},
  booktitle={2010 IEEE 71st Vehicular Technology Conference},
  pages={1--5},
  year={2010},
  organization={IEEE}
}

@inproceedings{xu2008narrowband,
  title={Narrowband interference suppression using RKF-based recurrent neural network in spread spectrum system},
  author={Xu, Ding-Jie and Zhao, Pi-Jie and Shen, Feng and Zhao, Hong},
  booktitle={2008 4th International Conference on Wireless Communications, Networking and Mobile Computing},
  pages={1--5},
  year={2008},
  organization={IEEE}
}

@article{wang2021cfar,
  title={CFAR-Based Interference Mitigation for FMCW Automotive Radar Systems},
  author={Wang, Jianping},
  journal={arXiv preprint arXiv:2101.01257},
  year={2021}
}

@book{richards2005fundamentals,
  title={Fundamentals of radar signal processing},
  author={Richards, Mark A},
  year={2005},
  publisher={Tata McGraw-Hill Education}
}

@article{alland2019interference,
  title={Interference in automotive radar systems: Characteristics, mitigation techniques, and current and future research},
  author={Alland, Stephen and Stark, Wayne and Ali, Murtaza and Hegde, Manju},
  journal={IEEE Signal Processing Magazine},
  volume={36},
  number={5},
  pages={45--59},
  year={2019},
  publisher={IEEE}
}

@article{chen2021coexistence,
  title={Coexistence and Interference Mitigation for {WPANs} and {WLANs} from Traditional Approaches to Deep Learning: A Review},
  author={Chen, Dong and Zhuang, Yuan and Huai, Jianzhu and Sun, Xiao and Yang, Xiansheng and Javed, Muhammad Awais and Brown, Jason and Sheng, Zhengguo and Thompson, John},
  journal={IEEE Sensors Journal},
  year={2021},
  publisher={IEEE}
}

@article{geng2021deep,
  title={Deep-Learning for Radar: A Survey},
  author={Geng, Zhe and Yan, He and Zhang, Jindong and Zhu, Daiyin},
  journal={IEEE Access},
  year={2021},
  publisher={IEEE}
}

@article{chang1999narrow,
  title={Narrow-band interference suppression in spread-spectrum {CDMA} communications using pipelined recurrent neural networks},
  author={Chang, Po-Rong and Hu, Jen-Tsung},
  journal={IEEE Transactions on Vehicular Technology},
  volume={48},
  number={2},
  pages={467--477},
  year={1999},
  publisher={IEEE}
}

@inproceedings{zhang2018self,
  title={A self-interference cancellation method based on deep learning for beyond 5G full-duplex system},
  author={Zhang, WeiMin and Yin, Jun and Wu, Di and Guo, Gan and Lai, Zhijing},
  booktitle={2018 IEEE International Conference on Signal Processing, Communications and Computing (ICSPCC)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@article{polak2011identifying,
  title={Identifying wireless users via transmitter imperfections},
  author={Polak, Adam C and Dolatshahi, Sepideh and Goeckel, Dennis L},
  journal={IEEE Journal on selected areas in communications},
  volume={29},
  number={7},
  pages={1469--1479},
  year={2011},
  publisher={IEEE}
}

@inproceedings{schmidt2017wireless,
  title={Wireless interference identification with convolutional neural networks},
  author={Schmidt, Malte and Block, Dimitri and Meier, Uwe},
  booktitle={2017 IEEE 15th International Conference on Industrial Informatics (INDIN)},
  pages={180--185},
  year={2017},
  organization={IEEE}
}

@article{yu2020interference,
  title={Interference Classification Using Deep Neural Networks},
  author={Yu, Jianyuan and Alhassoun, Mohammad and Buehrer, R Michael},
  journal={arXiv preprint arXiv:2002.00533},
  year={2020}
}

@misc{matlab,
  title = {{CWT}-Based Time-Frequency Analysis},
  howpublished = {\url{https://www.mathworks.com/help/wavelet/examples/cwt-based-time-frequency-analysis.html}},
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{meng2017research,
  title={Research on denoising sparse autoencoder},
  author={Meng, Lingheng and Ding, Shifei and Xue, Yu},
  journal={International Journal of Machine Learning and Cybernetics},
  volume={8},
  number={5},
  pages={1719--1729},
  year={2017},
  publisher={Springer}
}

@article{wang2016auto,
  title={Auto-encoder based dimensionality reduction},
  author={Wang, Yasi and Yao, Hongxun and Zhao, Sicheng},
  journal={Neurocomputing},
  volume={184},
  pages={232--242},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{zhou2017anomaly,
  title={Anomaly detection with robust deep autoencoders},
  author={Zhou, Chong and Paffenroth, Randy C},
  booktitle={Proceedings of the 23rd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={665--674},
  year={2017}
}

@inproceedings{shcherbakov2014image,
  title={Image inpainting based on stacked autoencoders},
  author={Shcherbakov, O and Batishcheva, V},
  booktitle={Journal of Physics: Conference Series},
  volume={536},
  pages={012020},
  year={2014},
  organization={IOP Publishing}
}

@article{gascon2009security,
  title={Security in 802.15. 4 and {ZigBee} networks},
  author={Gasc{\'o}n, David},
  journal={Apr},
  volume={28},
  pages={1--5},
  year={2009}
}

@article{lu2006survey,
  title={Survey on interference mitigation via adaptive array processing in {GPS}},
  author={Lu, Dan and Feng, Qing and Wu, Renbiao},
  journal={Piers Online},
  volume={2},
  number={4},
  pages={357--362},
  year={2006},
  publisher={PIERS Online}
}

@article{le2015interference,
  title={Interference mitigation schemes for wireless body area sensor networks: A comparative survey},
  author={Le, Thien TT and Moh, Sangman},
  journal={Sensors},
  volume={15},
  number={6},
  pages={13805--13838},
  year={2015},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{chang2006digital,
  title={Digital {GFSK} carrier synchronization},
  author={Chang, Dah-Chung and Shiu, Tsung-Hau},
  booktitle={APCCAS 2006-2006 IEEE Asia Pacific Conference on Circuits and Systems},
  pages={1523--1526},
  year={2006},
  organization={IEEE}
}

@inproceedings{tjensvold2007comparison,
  title={Comparison of the {IEEE} 802.11, 802.15. 1, 802.15. 4 and 802.15. 6 wireless standards},
  author={Tjensvold, Jan Magne},
  booktitle={IEEE: September},
  volume={18},
  year={2007}
}

@misc{wiki:Error_vector_magnitude,
   author = "Wikipedia",
   title = "{Error vector magnitude} --- {W}ikipedia{,} The Free Encyclopedia",
   year = "2021",
   howpublished = {\url{http://en.wikipedia.org/w/index.php?title=Error\%20vector\%20magnitude&oldid=984897738}},
   note = "[Online; accessed 21-October-2021]"
 }

@article{gomez2012overview,
  title={Overview and evaluation of bluetooth low energy: An emerging low-power wireless technology},
  author={Gomez, Carles and Oller, Joaquim and Paradells, Josep},
  journal={Sensors},
  volume={12},
  number={9},
  pages={11734--11753},
  year={2012},
  publisher={Molecular Diversity Preservation International}
}

@article{slavivc2003damping,
  title={Damping identification using a continuous wavelet transform: application to real data},
  author={Slavi{\v{c}}, Janko and Simonovski, Igor and Bolte{\v{z}}ar, Miha},
  journal={Journal of Sound and Vibration},
  volume={262},
  number={2},
  pages={291--307},
  year={2003},
  publisher={Elsevier}
}

@article{pizurica2006estimating,
  title={Estimating the probability of the presence of a signal of interest in multiresolution single-and multiband image denoising},
  author={Pizurica, Aleksandra and Philips, Wilfried},
  journal={IEEE Transactions on image processing},
  volume={15},
  number={3},
  pages={654--665},
  year={2006},
  publisher={IEEE}
}

@inproceedings{feng2014cross,
  title={Cross-modal retrieval with correspondence autoencoder},
  author={Feng, Fangxiang and Wang, Xiaojie and Li, Ruifan},
  booktitle={Proceedings of the 22nd ACM International Conference on Multimedia},
  pages={7--16},
  year={2014}
}

@article{akeret2017radio,
  title={Radio frequency interference mitigation using deep convolutional neural networks},
  author={Akeret, Joel and Chang, Chihway and Lucchi, Aurelien and Refregier, Alexandre},
  journal={Astronomy and Computing},
  volume={18},
  pages={35--39},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{mun2018deep,
  title={A deep learning approach for automotive radar interference mitigation},
  author={Mun, Jiwoo and Kim, Heasung and Lee, Jungwoo},
  booktitle={2018 IEEE 88th Vehicular Technology Conference (VTC-Fall)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@article{ristea2020fully,
  title={Fully convolutional neural networks for automotive radar interference mitigation},
  author={Ristea, Nicolae-C{\u{a}}t{\u{a}}lin and Anghel, Andrei and Ionescu, Radu Tudor},
  journal={arXiv preprint arXiv:2007.11102},
  year={2020}
}

@inproceedings{fuchs2020automotive,
  title={Automotive Radar Interference Mitigation using a Convolutional Autoencoder},
  author={Fuchs, Jonas and Dubey, Anand and L{\"u}bke, Maximilian and Weigel, Robert and Lurz, Fabian},
  booktitle={2020 IEEE International Radar Conference (RADAR)},
  pages={315--320},
  year={2020},
  organization={IEEE}
}

@article{uysal2018synchronous,
  title={Synchronous and asynchronous radar interference mitigation},
  author={Uysal, Faruk},
  journal={IEEE Access},
  volume={7},
  pages={5846--5852},
  year={2018},
  publisher={IEEE}
}

@article{fabrizio2014blind,
  title={Blind source separation with the generalised estimation of multipath signals algorithm},
  author={Fabrizio, Giuseppe and Farina, Alfonso},
  journal={IET Radar, Sonar \& Navigation},
  volume={8},
  number={9},
  pages={1255--1266},
  year={2014},
  publisher={IET}
}

@article{breed2003bit,
  title={Bit error rate: Fundamental concepts and measurement issues},
  author={Breed, Gary},
  journal={High Frequency Electronics},
  volume={2},
  number={1},
  pages={46--47},
  year={2003},
  publisher={Summit Technical Media}
}

@article{li2016dme,
  title={{DME} interference suppression algorithm based on signal separation estimation theory for civil aviation system},
  author={Li, Jie and Wu, Renbiao and Hao, Yun and Wang, Xihua and Wang, Yali and Zhao, An},
  journal={EURASIP Journal on Wireless Communications and Networking},
  volume={2016},
  number={1},
  pages={1--8},
  year={2016},
  publisher={Springer}
}

@article{johnson2006signal,
  title={Signal-to-noise ratio},
  author={Johnson, Don H},
  journal={Scholarpedia},
  volume={1},
  number={12},
  pages={2088},
  year={2006}
}

@article{haenggi2009stochastic,
  title={Stochastic geometry and random graphs for the analysis and design of wireless networks},
  author={Haenggi, Martin and Andrews, Jeffrey G and Baccelli, Fran{\c{c}}ois and Dousse, Olivier and Franceschetti, Massimo},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={27},
  number={7},
  pages={1029--1046},
  year={2009},
  publisher={IEEE}
}

@article{jeruchim1984techniques,
  title={Techniques for estimating the bit error rate in the simulation of digital communication systems},
  author={Jeruchim, Michel},
  journal={IEEE Journal on selected areas in communications},
  volume={2},
  number={1},
  pages={153--170},
  year={1984},
  publisher={IEEE}
}

@article{fan2019interference,
  title={Interference mitigation for synthetic aperture radar based on deep residual network},
  author={Fan, Weiwei and Zhou, Feng and Tao, Mingliang and Bai, Xueru and Rong, Pengshuai and Yang, Shuang and Tian, Tian},
  journal={Remote Sensing},
  volume={11},
  number={14},
  pages={1654},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{xu2018deep,
  title={Deep learning for interference cancellation in non-orthogonal signal based optical communication systems},
  author={Xu, Tongyang and Xu, Tianhua and Darwazeh, Izzat},
  booktitle={2018 Progress in Electromagnetics Research Symposium (PIERS-Toyama)},
  pages={241--248},
  year={2018},
  organization={IEEE}
}

@inproceedings{rock2019complex,
  title={Complex signal denoising and interference mitigation for automotive radar using convolutional neural networks},
  author={Rock, Johanna and Toth, Mate and Messner, Elmar and Meissner, Paul and Pernkopf, Franz},
  booktitle={2019 22th International Conference on Information Fusion (FUSION)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@article{rock2020quantized,
  title={Quantized Neural Networks for Radar Interference Mitigation},
  author={Rock, Johanna and Roth, Wolfgang and Toth, Mate and Meissner, Paul and Pernkopf, Franz},
  journal={arXiv preprint arXiv:2011.12706},
  year={2020}
}

@techreport{gardner1994cyclostationarity,
  title={Cyclostationarity in communications and signal processing},
  author={Gardner, William A},
  year={1994},
  institution={STATISTICAL SIGNAL PROCESSING INC YOUNTVILLE CA}
}

@article{reed1995optimal,
  title={An optimal receiver using a time-dependent adaptive filter},
  author={Reed, Jeffrey H and Yuen, NM and Hsia, Tien C},
  journal={IEEE Transactions on Communications},
  volume={43},
  number={2/3/4},
  pages={187--190},
  year={1995},
  publisher={IEEE}
}

@article{zhang1999blind,
  title={Blind adaptive FRESH filtering for signal extraction},
  author={Zhang, J and Wong, Kon Max and Luo, ZQ and Ching, PC},
  journal={IEEE Transactions on Signal Processing},
  volume={47},
  number={5},
  pages={1397--1402},
  year={1999},
  publisher={IEEE}
}

@article{grunau2018multi,
  title={Multi-label wireless interference identification with convolutional neural networks},
  author={Grunau, Sergej and Block, Dimitri and Meier, Uwe},
  journal={arXiv preprint arXiv:1804.04395},
  year={2018}
}

@article{o2017introduction,
  title={An introduction to deep learning for the physical layer},
  author={O’Shea, Timothy and Hoydis, Jakob},
  journal={IEEE Transactions on Cognitive Communications and Networking},
  volume={3},
  number={4},
  pages={563--575},
  year={2017},
  publisher={IEEE}
}

@article{ujan2020efficient,
  AUTHOR = {Ujan, Sahar and Navidi, Neda and Jr Landry, Rene},
TITLE = {An Efficient Radio Frequency Interference ({RFI}) Recognition and Characterization Using End-to-End Transfer Learning},
JOURNAL = {Applied Sciences},
VOLUME = {10},
YEAR = {2020},
NUMBER = {19},
ARTICLE-NUMBER = {6885},
URL = {https://www.mdpi.com/2076-3417/10/19/6885},
ISSN = {2076-3417},
}

@inproceedings{kim2007cyclostationary,
  title={Cyclostationary approaches to signal detection and classification in cognitive radio},
  author={Kim, Kyouwoong and Akbar, Ihsan A and Bae, Kyung K and Um, Jung-Sun and Spooner, Chad M and Reed, Jeffrey H},
  booktitle={2007 2nd {IEEE} International Symposium on New Frontiers in Dynamic Spectrum Access Networks},
  pages={212--215},
  year={2007},
  organization={IEEE}
}

@inproceedings{shahid2019convolutional,
  title={A convolutional neural network approach for classification of {LPWAN} technologies: {Sigfox}, {LORA} and {IEEE} 802.15. 4g},
  author={Shahid, Adnan and Fontaine, Jaron and Camelo, Miguel and Haxhibeqiri, Jetmir and Saelens, Martijn and Khan, Zaheer and Moerman, Ingrid and De Poorter, Eli},
  booktitle={2019 16th Annual IEEE International Conference on Sensing, Communication, and Networking (SECON)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@inproceedings{batra2006mitigation,
  title={Mitigation of narrowband interference using adaptive equalizers},
  author={Batra, Arun and Zeidler, James R and Beex, AA},
  booktitle={2006 14th European Signal Processing Conference},
  pages={1--5},
  year={2006},
  organization={IEEE}
}

@inproceedings{hithnawi2014understanding,
  title={Understanding the impact of cross technology interference on {IEEE} 802.15. 4},
  author={Hithnawi, Anwar and Shafagh, Hossein and Duquennoy, Simon},
  booktitle={Proceedings of the 9th ACM international workshop on Wireless network testbeds, experimental evaluation and characterization},
  pages={49--56},
  year={2014}
}

@inproceedings{hithnawi2016crosszig,
  title={Crosszig: combating cross-technology interference in low-power wireless networks},
  author={Hithnawi, Anwar and Li, Su and Shafagh, Hossein and Gross, James and Duquennoy, Simon},
  booktitle={2016 15th ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)},
  pages={1--12},
  year={2016},
  organization={IEEE}
}

@inproceedings{wang2021prcomm,
  title={{PRComm}: Anti-Interference Cross-Technology Communication Based on Pseudo-random Sequence},
  author={Wang, Wei and He, Dingsheng and Jia, Wan and Chen, Xiaojiang and Gu, Tao and Liu, Haiyan and Sun, Xiaoyang and Chen, Guannan and Wu, Fuping},
  booktitle={Proceedings of the 20th International Conference on Information Processing in Sensor Networks (co-located with CPS-IoT Week 2021)},
  pages={163--175},
  year={2021}
}

@inproceedings{ahmad2010neuro,
  title={Neuro-fuzzy signal classifier (NFSC) for standard wireless technologies},
  author={Ahmad, Kaleem and Shresta, Ganesh and Meier, Uwe and Kwasnicka, Halina},
  booktitle={2010 7th International Symposium on Wireless Communication Systems},
  pages={616--620},
  year={2010},
  organization={IEEE}
}

@inproceedings{longi2017semi,
  title={Semi-supervised convolutional neural networks for identifying {Wi-Fi} interference sources},
  author={Longi, Krista and Pulkkinen, Teemu and Klami, Arto},
  booktitle={Asian Conference on Machine Learning},
  pages={391--406},
  year={2017},
  organization={PMLR}
}

@article{lynggaard2018using,
  title={Using machine learning for adaptive interference suppression in wireless sensor networks},
  author={Lynggaard, Per},
  journal={IEEE Sensors Journal},
  volume={18},
  number={21},
  pages={8820--8826},
  year={2018},
  publisher={IEEE}
}

@article{suzain2020machine,
  title={Machine learning based lightweight interference mitigation scheme for wireless sensor network},
  author={Suzain, Ali and Rashid, Rozeha A and Sarijari, MA and Abdullah, A Shahidan and Aziz, Omar A},
  journal={Telkomnika},
  volume={18},
  number={4},
  pages={1762--1770},
  year={2020},
  publisher={Ahmad Dahlan University}
}

@article{hermans2012lightweight,
  title={A lightweight approach to online detection and classification of interference in 802.15.4-based sensor networks},
  author={Hermans, Frederik and Larzon, Lars-{\AA}ke and Rensfelt, Olof and Gunningberg, Per},
  journal={Acm Sigbed Review},
  volume={9},
  number={3},
  pages={11--20},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@inproceedings{wagner2018threshold,
  title={Threshold-free interference cancellation method for automotive {FMCW} radar systems},
  author={Wagner, Matthias and Sulejmani, Fisnik and Melzer, Alexander and Meissner, Paul and Huemer, Mario},
  booktitle={2018 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1--4},
  year={2018},
  organization={IEEE}
}

@article{narkhede2018understanding,
  title={Understanding auc-roc curve},
  author={Narkhede, Sarang},
  journal={Towards Data Science},
  volume={26},
  pages={220--227},
  year={2018}
}

@article{schmogrow2011error,
  title={Error vector magnitude as a performance measure for advanced modulation formats},
  author={Schmogrow, Rene and Nebendahl, Bernd and Winter, Marcus and Josten, Arne and Hillerkuss, David and Koenig, Swen and Meyer, Joachim and Dreschmann, Michael and Huebner, Michael and Koos, Christian and others},
  journal={IEEE Photonics Technology Letters},
  volume={24},
  number={1},
  pages={61--63},
  year={2011},
  publisher={IEEE}
}

@article{wang2004image,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P},
  journal={IEEE Transactions on Image Processing},
  volume={13},
  number={4},
  pages={600--612},
  year={2004},
  publisher={IEEE}
}

@inproceedings{bechter2017automotive,
  title={Automotive radar interference mitigation using a sparse sampling approach},
  author={Bechter, Jonathan and Roos, Fabian and Rahman, Mahfuzur and Waldschmidt, Christian},
  booktitle={2017 European Radar Conference (EURAD)},
  pages={90--93},
  year={2017},
  organization={IEEE}
}

@book {fischer2016untersuchungen,
  title = {Studies on the interference behavior of automotive radar sensors},
  author = {Fischer, Christoph},
  year = {2016},
  publisher = {Cuvillier Verlag}
}

@inproceedings{marvasti2012sparse,
  title={Sparse signal processing using iterative method with adaptive thresholding {(IMAT)}},
  author={Marvasti, Farrokh and Azghani, Masoume and Imani, P and Pakrouh, P and Heydari, Seyed Javad and Golmohammadi, Azarang and Kazerouni, A and Khalili, MM},
  booktitle={2012 19th International Conference on Telecommunications (ICT)},
  pages={1--6},
  year={2012},
  organization={IEEE}
}

@inproceedings{tullsson1997topics,
  title={Topics in {FMCW} radar disturbance suppression},
  author={Tullsson, B-E},
  booktitle={Radar 97 (Conf. Publ. No. 449)},
  pages={1--5},
  year={1997},
  organization={IET}
}

@article{chan1981parameter,
  title={A parameter estimation approach to estimation of frequencies of sinusoids},
  author={Chan, Y and Lavoie, J and Plant, J},
  journal={IEEE Transactions on Acoustics, Speech, and Signal Processing},
  volume={29},
  number={2},
  pages={214--219},
  year={1981},
  publisher={IEEE}
}

@inproceedings{yuan2010adaptive,
  title={Adaptive CCA for {IEEE} 802.15. 4 wireless sensor networks to mitigate interference},
  author={Yuan, Wei and Linnartz, Jean-Paul MG and Niemegeers, Ignas GMM},
  booktitle={2010 IEEE Wireless Communication and Networking Conference},
  pages={1--5},
  year={2010},
  organization={IEEE}
}

@inproceedings{vanheel2007spectral,
  title={Spectral interference study of {Wi-Fi} on wireless sensor networks},
  author={Vanheel, Frank and Moerman, Ingrid and Verhaevert, Jo},
  booktitle={8th UGent PhD symposium},
  pages={108--108},
  year={2007}
}

@inproceedings{chowdhury2009interferer,
  title={Interferer classification, channel selection and transmission adaptation for wireless sensor networks},
  author={Chowdhury, Kaushik R and Akyildiz, Ian F},
  booktitle={2009 IEEE International Conference on Communications},
  pages={1--5},
  year={2009},
  organization={IEEE}
}

@inproceedings{yoon2010adaptive,
  title={Adaptive channel hopping for interference robust wireless sensor networks},
  author={Yoon, S-U and Murawski, Robert and Ekici, Eylem and Park, Sangjoon and Mir, Zeeshan Hameed},
  booktitle={2010 IEEE International Conference on Communications},
  pages={1--5},
  year={2010},
  organization={IEEE}
}

@inproceedings{yun2008channel,
  title={A channel switching scheme for avoiding interference of between {IEEE} 802.15. 4 and other networks},
  author={Yun, Jangkyu and Lee, Byeongjik and Li, Jilong and Han, Kijun},
  booktitle={2008 International Multi-symposiums on Computer and Computational Sciences},
  pages={136--139},
  year={2008},
  organization={IEEE}
}

@inproceedings{hassan2013mitigating,
  title={Mitigating interference in a heterogeneous wireless network using channel selection},
  author={Hassan, MN and Kamarudin, LM and Zakaria, A},
  booktitle={Special Issue for International Conference of Advanced Materials Engineering and Technology},
  year={2013}
}

@inproceedings{hou2009minimizing,
  title={Minimizing 802.11 interference on zigbee medical sensors},
  author={Hou, James and Chang, Benjamin and Cho, Dae-Ki and Gerla, Mario},
  booktitle={Proceedings of the Fourth International Conference on Body Area Networks},
  pages={1--8},
  year={2009}
}

@inproceedings{du2012adaptive,
  title={Adaptive time slotted channel hopping for wireless sensor networks},
  author={Du, Peng and Roussos, George},
  booktitle={2012 4th Computer Science and Electronic Engineering Conference (CEEC)},
  pages={29--34},
  year={2012},
  organization={IEEE}
}

@inproceedings{toth2019performance,
  title={Performance comparison of mutual automotive radar interference mitigation algorithms},
  author={Toth, Mate and Meissner, Paul and Melzer, Alexander and Witrisal, Klaus},
  booktitle={2019 IEEE Radar Conference (RadarConf)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@inproceedings{hithnawi2013exploiting,
  title={Exploiting physical layer information to mitigate cross-technology interference effects on low-power wireless networks},
  author={Hithnawi, Anwar},
  booktitle={Proceedings of the 11th ACM Conference on Embedded Networked Sensor Systems},
  pages={1--2},
  year={2013}
}

@article{lipton2015critical,
  title={A critical review of recurrent neural networks for sequence learning},
  author={Lipton, Zachary C and Berkowitz, John and Elkan, Charles},
  journal={arXiv preprint arXiv:1506.00019},
  year={2015}
}

@inproceedings{lin2020cross,
  title={Cross-Technology Interference Mitigation Using Fully Convolutional Denoising Autoencoders},
  author={Lin, Chi-Lun and Lin, Kate Ching-Ju and Lee, Chi-Cheng and Tsao, Yu},
  booktitle={GLOBECOM 2020-2020 IEEE Global Communications Conference},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@inproceedings{zheng2020mitigating,
  title={Mitigating Cross-Technology Interference in Heterogeneous Wireless Networks based on Deep Learning},
  author={Zheng, Weidong and Yao, Junmei and Wu, Kaishun},
  booktitle={2020 IEEE 26th International Conference on Parallel and Distributed Systems (ICPADS)},
  pages={230--237},
  year={2020},
  organization={IEEE}
}

@article{doersch2016tutorial,
  title={Tutorial on variational autoencoders},
  author={Doersch, Carl},
  journal={arXiv preprint arXiv:1606.05908},
  year={2016}
}

@article{wang2019data,
  title={Data-driven deep learning for automatic modulation recognition in cognitive radios},
  author={Wang, Yu and Liu, Miao and Yang, Jie and Gui, Guan},
  journal={IEEE Transactions on Vehicular Technology},
  volume={68},
  number={4},
  pages={4074--4077},
  year={2019},
  publisher={IEEE}
}

@article{youssef2017machine,
  title={Machine Learning Approach to {RF} Transmitter Identification},
  author={Youssef, Khalid and Bouchard, Louis-S and Haigh, KZ and Krovi, H and Silovsky, J and Vander Valk, CP},
  journal={arXiv preprint arXiv:1711.01559},
  year={2017}
}

@article{aceto2019mobile,
  title={Mobile encrypted traffic classification using deep learning: Experimental evaluation, lessons learned, and challenges},
  author={Aceto, Giuseppe and Ciuonzo, Domenico and Montieri, Antonio and Pescap{\'e}, Antonio},
  journal={IEEE Transactions on Network and Service Management},
  volume={16},
  number={2},
  pages={445--458},
  year={2019},
  publisher={IEEE}
}

@inproceedings{liu2020distributed,
  title={Distributed and Accurate Packet Reception Rate Estimation under Cross-Technology Interference},
  author={Liu, Wei and Xia, Yu and Xu, Ming and Xie, Jian and Luo, Rong and Huang, Daqing},
  booktitle={GLOBECOM 2020-2020 IEEE Global Communications Conference},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@inproceedings{pulkkinen2020understanding,
  title={Understanding {Wi}-{Fi} cross-technology interference detection in the real world},
  author={Pulkkinen, Teemu and Nurminen, Jukka K and Nurmi, Petteri},
  booktitle={2020 IEEE 40th International Conference on Distributed Computing Systems (ICDCS)},
  pages={954--964},
  year={2020},
  organization={IEEE}
}

@article{kim2020classification,
  title={Classification of Interference Signal for Automotive Radar Systems With Convolutional Neural Network},
  author={Kim, Jinwook and Lee, Seongwook and Kim, Yong-Hwa and Kim, Seong-Cheol},
  journal={IEEE Access},
  volume={8},
  pages={176717--176727},
  year={2020},
  publisher={IEEE}
}

@misc{deepsig,
  title={{RF} Datasets for Machine Learning},
  howpublished = {\url{https://www.deepsig.ai/datasets}},
}

@article{kussul2004improved,
  title={Improved method of handwritten digit recognition tested on {MNIST} database},
  author={Kussul, Ernst and Baidyk, Tatiana},
  journal={Image and Vision Computing},
  volume={22},
  number={12},
  pages={971--981},
  year={2004},
  publisher={Elsevier}
}

@inproceedings{cohen2017emnist,
  title={{EMNIST}: Extending MNIST to handwritten letters},
  author={Cohen, Gregory and Afshar, Saeed and Tapson, Jonathan and Van Schaik, Andre},
  booktitle={2017 International Joint Conference on Neural Networks (IJCNN)},
  pages={2921--2926},
  year={2017},
  organization={IEEE}
}

@misc{crawdad,
  title={{CRAWDAD} A Community Resource for Archiving Wireless Data at Dartmouth},
  howpublished = {\url{https://crawdad.org/}},
}

@misc{rutgers-noise-20070420,
    author = {Sanjit Krishnan Kaul and Ivan Seskar and Marco Gruteser},
    title = {{CRAWDAD} dataset rutgers/noise (v. 2007-04-20)},
    howpublished = {Downloaded from \url{https://crawdad.org/rutgers/noise/20070420/RSSI}},
    note = {traceset: RSSI},
    doi = {10.15783/C7B59W},
    month = apr,
    year = 2007
}

@misc{kyutech-interference-20150616,
    author = {Marat Zhanikeev},
    title = {{CRAWDAD} dataset kyutech/interference (v. 2015-06-16)},
    howpublished = {Downloaded from \url{https://crawdad.org/kyutech/interference/20150616}},
    doi = {10.15783/C7T88W},
    month = jun,
    year = 2015
}

@misc{owl-interference-20190212,
    author = {Malte Schmidt and Dimitri Block and Uwe Meier},
    title = {{CRAWDAD} dataset {OWL}/interference (v. 2019-02-12)},
    howpublished = {Downloaded from \url{https://crawdad.org/owl/interference/20190212}},
    month = feb,
    year = 2019
}

@article{grimaldi2018real,
  title={Real-time interference identification via supervised learning: Embedding coexistence awareness in {IoT} devices},
  author={Grimaldi, Simone and Mahmood, Aamir and Gidlund, Mikael},
  journal={IEEE Access},
  volume={7},
  pages={835--850},
  year={2018},
  publisher={IEEE}
}

@inproceedings{o2016convolutional,
  title={Convolutional radio modulation recognition networks},
  author={O’Shea, Timothy J and Corgan, Johnathan and Clancy, T Charles},
  booktitle={International conference on engineering applications of neural networks},
  pages={213--226},
  year={2016},
  organization={Springer}
}

@article{yang2003co,
  title={Co-channel interference modeling and analysis in a Poisson field of interferers in wireless communications},
  author={Yang, Xueshi and Petropulu, Athina P},
  journal={IEEE Transactions on signal processing},
  volume={51},
  number={1},
  pages={64--76},
  year={2003},
  publisher={IEEE}
}

@inproceedings{kajita2016wi,
  title={{Wi}-{Fi} channel selection based on urban interference measurement},
  author={Kajita, Shugo and Amano, Tatsuya and Yamaguchi, Hirozumi and Higashino, Teruo and Takai, Mineo},
  booktitle={Proceedings of the 13th International Conference on Mobile and Ubiquitous Systems: Computing, Networking and Services},
  pages={143--150},
  year={2016}
}

@article{milstein1988interference,
  title={Interference rejection techniques in spread spectrum communications},
  author={Milstein, Laurence B},
  journal={Proceedings of the IEEE},
  volume={76},
  number={6},
  pages={657--671},
  year={1988},
  publisher={IEEE}
}

@article{vijayan1990nonlinear,
  title={Nonlinear techniques for interference suppression in spread-spectrum systems},
  author={Vijayan, Rajiv and Poor, H Vincent},
  journal={IEEE Transactions on Communications},
  volume={38},
  number={7},
  pages={1060--1065},
  year={1990},
  publisher={IEEE}
}

@article{zhai2018energy,
  title={Energy-efficient user scheduling and power allocation for {NOMA-based} wireless networks with massive {IoT} devices},
  author={Zhai, Daosen and Zhang, Ruonan and Cai, Lin and Li, Bin and Jiang, Yi},
  journal={IEEE Internet of Things Journal},
  volume={5},
  number={3},
  pages={1857--1868},
  year={2018},
  publisher={IEEE}
}

@inproceedings{hasan2020role,
  title={The role of deep learning in NOMA for {5G} and beyond communications},
  author={Hasan, Moh Khalid and Shahjalal, Md and Islam, Md Mainul and Alam, Md Morshed and Ahmed, Md Faisal and Jang, Yeong Min},
  booktitle={2020 International Conference on Artificial Intelligence in Information and Communication (ICAIIC)},
  pages={303--307},
  year={2020},
  organization={IEEE}
}

@inproceedings{azmi2014interference,
  title={Interference issues and mitigation method in WSN 2.4 {GHz} {ISM} band: A survey},
  author={Azmi, N and Kamarudin, LM and Mahmuddin, Massudi and Zakaria, Azizi and Shakaff, AYM and Khatun, S and Kamarudin, K and Morshed, MN},
  booktitle={2014 2nd International Conference on Electronic Design (ICED)},
  pages={403--408},
  year={2014},
  organization={IEEE}
}

@article{dorner2017deep,
  title={Deep learning based communication over the air},
  author={D{\"o}rner, Sebastian and Cammerer, Sebastian and Hoydis, Jakob and Ten Brink, Stephan},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={12},
  number={1},
  pages={132--143},
  year={2017},
  publisher={IEEE}
}

@article{wu2020deep,
  title={Deep Learning-Based Autoencoder for {m-User} Wireless Interference Channel Physical Layer Design},
  author={Wu, Dehao and Nekovee, Maziar and Wang, Yue},
  journal={IEEE Access},
  volume={8},
  pages={174679--174691},
  year={2020},
  publisher={IEEE}
}

@article{wu2019adaptive,
  title={An adaptive deep learning algorithm based autoencoder for interference channels},
  author={Wu, Dehao and Nekovee, Maziar and Wang, Yue},
  journal={arXiv preprint arXiv:1902.06841},
  year={2019}
}

@article{kunert2010d1,
  title={D1. 5-study on the state-of-the-art interference mitigation techniques},
  author={Kunert, M and Bodereau, F and Goppelt, M and Fischer, C and John, A and Wixforth, T and Ossowska, A and Schipper, T and others},
  year={2010},
  journal={Technical report, European Commission: MOre Safety for All by Radar}
}

@inproceedings{o2017physical,
  title={Physical layer deep learning of encodings for the {MIMO} fading channel},
  author={O'Shea, Timothy J and Erpek, Tugba and Clancy, T Charles},
  booktitle={2017 55th Annual Allerton Conference on Communication, Control, and Computing (Allerton)},
  pages={76--80},
  year={2017},
  organization={IEEE}
}

@inproceedings{o2018physical,
  title={Physical layer communications system design over-the-air using adversarial networks},
  author={O'Shea, Timothy J and Roy, Tamoghna and West, Nathan and Hilburn, Benjamin C},
  booktitle={2018 26th European Signal Processing Conference (EUSIPCO)},
  pages={529--532},
  year={2018},
  organization={IEEE}
}

@inproceedings{ye2018channel,
  title={Channel agnostic end-to-end learning based communication systems with conditional GAN},
  author={Ye, Hao and Li, Geoffrey Ye and Juang, Biing-Hwang Fred and Sivanesan, Kathiravetpillai},
  booktitle={2018 IEEE Globecom Workshops (GC Wkshps)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@article{ye2017power,
  title={Power of deep learning for channel estimation and signal detection in {OFDM} systems},
  author={Ye, Hao and Li, Geoffrey Ye and Juang, Biing-Hwang},
  journal={IEEE Wireless Communications Letters},
  volume={7},
  number={1},
  pages={114--117},
  year={2017},
  publisher={IEEE}
}

@article{o2015introduction,
  title={An introduction to convolutional neural networks},
  author={O'Shea, Keiron and Nash, Ryan},
  journal={arXiv preprint arXiv:1511.08458},
  year={2015}
}

@inproceedings{farid2016homogeneous,
  title={Homogeneous interference mitigation techniques for wireless body area network under coexistence: A survey},
  author={Farid, Sajid and Zia, Yousaf and Farhad, Arshad and Hussain, Faisal Bashir},
  booktitle={2016 IEEE Asia Pacific Conference on Wireless and Mobile (APWiMob)},
  pages={124--129},
  year={2016},
  organization={IEEE}
}

@article{liang2018iterative,
  title={An iterative {BP-CNN} architecture for channel decoding},
  author={Liang, Fei and Shen, Cong and Wu, Feng},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={12},
  number={1},
  pages={144--159},
  year={2018},
  publisher={IEEE}
}

@inproceedings{erpek2018learning,
  title={Learning a physical layer scheme for the {MIMO} interference channel},
  author={Erpek, Tugba and O'Shea, Timothy J and Clancy, T Charles},
  booktitle={2018 IEEE International Conference on Communications (ICC)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@article{nabil2015recent,
  title={Recent advances in interference management for wireless networks},
  author={Nabil, Amr and Hou, Y Thomas and Zhu, Rongbo and Lou, Wenjing and Midkiff, Scott F},
  journal={IEEE Network},
  volume={29},
  number={5},
  pages={83--89},
  year={2015},
  publisher={IEEE}
}

@inproceedings{o2016radio,
  title={Radio machine learning dataset generation with gnu radio},
  author={O'shea, Timothy J and West, Nathan},
  booktitle={Proceedings of the GNU Radio Conference},
  volume={1},
  number={1},
  year={2016}
}

@article{carrick2018paramorphic,
  title={Paramorphic multicarrier communications for interference mitigation},
  author={Carrick, Matt and Reed, Jeffrey H and Spooner, Chad M},
  journal={EURASIP Journal on Advances in Signal Processing},
  volume={2018},
  number={1},
  pages={1--18},
  year={2018},
  publisher={Springer}
}

@article{mitola1999cognitive,
  title={Cognitive radio: making software radios more personal},
  author={Mitola, Joseph and Maguire, Gerald Q},
  journal={IEEE personal communications},
  volume={6},
  number={4},
  pages={13--18},
  year={1999},
  publisher={IEEE}
}

@inproceedings{ciregan2012multi,
  title={Multi-column deep neural networks for image classification},
  author={Ciregan, Dan and Meier, Ueli and Schmidhuber, J{\"u}rgen},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3642--3649},
  year={2012},
  organization={IEEE}
}

@article{mireshghallah2020privacy,
  title={Privacy in deep learning: A survey},
  author={Mireshghallah, Fatemehsadat and Taram, Mohammadkazem and Vepakomma, Praneeth and Singh, Abhishek and Raskar, Ramesh and Esmaeilzadeh, Hadi},
  journal={arXiv preprint arXiv:2004.12254},
  year={2020}
}

@book{comon2010handbook,
  title={Handbook of Blind Source Separation: Independent component analysis and applications},
  author={Comon, Pierre and Jutten, Christian},
  year={2010},
  publisher={Academic press}
}

@misc{watanabe2007interference,
  title={Interference determination method and {FMCW} radar using the same},
  author={Watanabe, Yuu and Natsume, Kazuma},
  year={2007},
  month=mar # "~6",
  publisher={Google Patents},
  note={US Patent 7,187,321}
}

@article{fabrizio2011adaptive,
  title={An adaptive filtering algorithm for blind waveform estimation in diffuse multipath channels},
  author={Fabrizio, G and Farina, A},
  journal={IET Radar, Sonar \& Navigation},
  volume={5},
  number={3},
  pages={322--330},
  year={2011},
  publisher={IET}
}

@book{goodfellow2016deep,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}

@book{sutton2018reinforcement,
  title={Reinforcement learning: An introduction},
  author={Sutton, Richard S and Barto, Andrew G},
  year={2018},
  publisher={MIT press}
}

@inproceedings{caruana2006empirical,
  title={An empirical comparison of supervised learning algorithms},
  author={Caruana, Rich and Niculescu-Mizil, Alexandru},
  booktitle={Proceedings of the 23rd international conference on Machine learning},
  pages={161--168},
  year={2006}
}

@inproceedings{bengio2012deep,
  title={Deep learning of representations for unsupervised and transfer learning},
  author={Bengio, Yoshua},
  booktitle={Proceedings of ICML workshop on unsupervised and transfer learning},
  pages={17--36},
  year={2012},
  organization={JMLR Workshop and Conference Proceedings}
}

@incollection{hastie2009overview,
  title={Overview of supervised learning},
  author={Hastie, Trevor and Tibshirani, Robert and Friedman, Jerome},
  booktitle={The elements of statistical learning},
  pages={9--41},
  year={2009},
  publisher={Springer}
}

@phdthesis{agee1989property,
  title={The property-restoral approach to blind adaptive signal extraction},
  author={Agee, Brian Grant},
  year={1989},
  school={University of California, Davis}
}

@inproceedings{fite1996blind,
  title={Blind separation of voice modulated single-side-band using the multi-target variable modulus algorithm},
  author={Fite, John D and Bruzzone, Stephen P and Agee, Brian G},
  booktitle={1996 IEEE International Conference on Acoustics, Speech, and Signal Processing Conference Proceedings},
  volume={5},
  pages={2726--2729},
  year={1996},
  organization={IEEE}
}

@inproceedings{agee1993simulation,
  title={Simulation performance of a blind adaptive array for a realistic mobile channel},
  author={Agee, Brian G and Reed, JH and Cohen, K and Hsia, Tien C},
  booktitle={IEEE 43rd Vehicular Technology Conference},
  pages={97--100},
  year={1993},
  organization={IEEE}
}

@article{standard1996telecommunications,
  title={Telecommunications: Glossary of telecommunication terms},
  author={Standard, Federal and others},
  journal={Retrieved January},
  volume={15},
  number={2004},
  pages={69--72},
  year={1996}
}

@inproceedings{albawi2017understanding,
  title={Understanding of a convolutional neural network},
  author={Albawi, Saad and Mohammed, Tareq Abed and Al-Zawi, Saad},
  booktitle={2017 International Conference on Engineering and Technology (ICET)},
  pages={1--6},
  year={2017},
  organization={IEEE}
}

@article{hu2012interference,
  title={Interference avoidance for in-device coexistence in {3GPP} {LTE}-advanced: Challenges and solutions},
  author={Hu, Zhenping and Susitaival, Riikka and Chen, Zhuo and Fu, I-Kang and Dayal, Pranav and Baghel, Sudhir Kumar},
  journal={IEEE Communications Magazine},
  volume={50},
  number={11},
  pages={60--67},
  year={2012},
  publisher={IEEE}
}

@article{bayhan2017coexistence,
  title={Coexistence gaps in space: Cross-technology interference-nulling for improving {LTE-U}/{Wi}-{Fi} coexistence},
  author={Bayhan, Suzan and Zubow, Anatolij and Wolisz, Adam},
  journal={arXiv preprint arXiv:1710.07927},
  year={2017}
}

@article{naik2018coexistence,
  title={Coexistence of wireless technologies in the 5 {GHz} bands: A survey of existing solutions and a roadmap for future research},
  author={Naik, Gaurang and Liu, Jinshan and Park, Jung-Min Jerry},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={20},
  number={3},
  pages={1777--1798},
  year={2018},
  publisher={IEEE}
}

@article{chen2016coexistence,
  title={Coexistence of {LTE-LAA} and {Wi}-{Fi} on 5 {GHz} with corresponding deployment scenarios: A survey},
  author={Chen, Bolin and Chen, Jiming and Gao, Yuan and Zhang, Jie},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={19},
  number={1},
  pages={7--32},
  year={2016},
  publisher={IEEE}
}

@inproceedings{tercero2011impact,
  title={Impact of aggregate interference on meteorological radar from secondary users},
  author={Tercero, Miurel and Sung, Ki Won and Zander, Jens},
  booktitle={2011 IEEE Wireless Communications and Networking Conference},
  pages={2167--2172},
  year={2011},
  organization={IEEE}
}

@inproceedings{lansford2013coexistence,
  title={Coexistence of unlicensed devices with {DSRC} systems in the 5.9 {GHz} ITS band},
  author={Lansford, Jim and Kenney, John B and Ecclesine, Peter},
  booktitle={2013 IEEE Vehicular Networking Conference},
  pages={9--16},
  year={2013},
  organization={IEEE}
}

@article{kenney2011dedicated,
  title={Dedicated short-range communications ({DSRC}) standards in the United States},
  author={Kenney, John B},
  journal={Proceedings of the IEEE},
  volume={99},
  number={7},
  pages={1162--1182},
  year={2011},
  publisher={IEEE}
}

@inproceedings{naik2017coexistence,
  title={Coexistence of dedicated short range communications ({DSRC}) and {Wi}-{Fi}: Implications to {Wi}-{Fi} performance},
  author={Naik, Gaurang and Liu, Jinshan and Park, Jung-Min Jerry},
  booktitle={IEEE INFOCOM 2017-IEEE Conference on Computer Communications},
  pages={1--9},
  year={2017},
  organization={IEEE}
}

@article{ali2017non,
  title={Non-orthogonal multiple access for large-scale {5G} networks: Interference aware design},
  author={Ali, Konpal Shaukat and Elsawy, Hesham and Chaaban, Anas and Alouini, Mohamed-Slim},
  journal={IEEE Access},
  volume={5},
  pages={21204--21216},
  year={2017},
  publisher={IEEE}
}

@article{wang2018optimal,
  title={Optimal distributed interference mitigation for small cell networks with non-orthogonal multiple access: A locally cooperative game},
  author={Wang, Xianling and Zhang, Haijun and Tian, Yue and Zhu, Chen and Leung, Victor CM},
  journal={IEEE Access},
  volume={6},
  pages={63107--63119},
  year={2018},
  publisher={IEEE}
}

@article{saltikoff2016threat,
  title={The threat to weather radars by wireless technology},
  author={Saltikoff, Elena and Cho, John YN and Tristant, Philippe and Huuskonen, Asko and Allmon, Lynn and Cook, Russell and Becker, Erik and Joe, Paul},
  journal={Bulletin of the American Meteorological Society},
  volume={97},
  number={7},
  pages={1159--1167},
  year={2016},
  publisher={American Meteorological Society}
}

@article{cao1996general,
  title={General approach to blind source separation},
  author={Cao, Xi-Ren and Liu, Ruey-wen},
  journal={IEEE Transactions on signal Processing},
  volume={44},
  number={3},
  pages={562--571},
  year={1996},
  publisher={IEEE}
}

@article{zhu2009introduction,
  title={Introduction to semi-supervised learning},
  author={Zhu, Xiaojin and Goldberg, Andrew B},
  journal={Synthesis Lectures on Artificial Intelligence and Machine Learning},
  volume={3},
  number={1},
  pages={1--130},
  year={2009},
  publisher={Morgan \& Claypool Publishers}
}

@article{chapelle2009semi,
  title={Semi-supervised learning (chapelle, o. et al., eds.; 2006)[book reviews]},
  author={Chapelle, Olivier and Scholkopf, Bernhard and Zien, Alexander},
  journal={IEEE Transactions on Neural Networks},
  volume={20},
  number={3},
  pages={542--542},
  year={2009},
  publisher={IEEE}
}

@article{berthelot2019mixmatch,
  title={Mixmatch: A holistic approach to semi-supervised learning},
  author={Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin},
  journal={arXiv preprint arXiv:1905.02249},
  year={2019}
}

@article{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Advances in Neural Information Processing Systems},
  volume={27},
  year={2014}
}

@article{ghannam2018sefdm,
  title={{SEFDM} over satellite systems with advanced interference cancellation},
  author={Ghannam, Hedaia and Darwazeh, Izzat},
  journal={IET Communications},
  volume={12},
  number={1},
  pages={59--66},
  year={2018},
  publisher={IET}
}

@article{kesteven2005adaptive,
  title={Adaptive filters revisited: Radio frequency interference mitigation in pulsar observations},
  author={Kesteven, M and Hobbs, G and Clement, R and Dawson, B and Manchester, R and Uppal, T},
  journal={Radio science},
  volume={40},
  number={5},
  year={2005},
  publisher={Wiley Online Library}
}

@inproceedings{mohammed2021interference,
  title={Interference Mitigation in the Wireless Communication Systems Using Adaptive Filters},
  author={Mohammed, Jafar Ramadhan},
  booktitle={IOP Conference Series: Materials Science and Engineering},
  volume={1152},
  pages={012001},
  year={2021},
  organization={IOP Publishing}
}

@article{farhang2011ofdm,
  title={{OFDM} versus filter bank multicarrier},
  author={Farhang-Boroujeny, Behrouz},
  journal={IEEE signal processing magazine},
  volume={28},
  number={3},
  pages={92--112},
  year={2011},
  publisher={IEEE}
}

@article{liu2020privacy,
  title={Privacy and security issues in deep learning: a survey},
  author={Liu, Ximeng and Xie, Lehui and Wang, Yaopeng and Zou, Jian and Xiong, Jinbo and Ying, Zuobin and Vasilakos, Athanasios V},
  journal={IEEE Access},
  volume={9},
  pages={4566--4593},
  year={2020},
  publisher={IEEE}
}

@inproceedings{carrick2017optimal,
  title={An optimal filter for signals with time-varying cyclostationary statistics},
  author={Carrick, Matt and Reed, Jeffrey H and Harris, Fred},
  booktitle={2017 22nd International Conference on Digital Signal Processing (DSP)},
  pages={1--5},
  year={2017},
  organization={IEEE}
}

@inproceedings{khawar2014spectrum,
  title={Spectrum sharing between S-band radar and {LTE} cellular system: A spatial approach},
  author={Khawar, Awais and Abdel-Hadi, Ahmed and Clancy, T Charles},
  booktitle={2014 IEEE International Symposium on Dynamic Spectrum Access Networks (DYSPAN)},
  pages={7--14},
  year={2014},
  organization={IEEE}
}

@article{mahal2017spectral,
  title={Spectral coexistence of {MIMO} radar and {MIMO} cellular system},
  author={Mahal, Jasmin A and Khawar, Awais and Abdelhadi, Ahmed and Clancy, T Charles},
  journal={IEEE Transactions on Aerospace and Electronic Systems},
  volume={53},
  number={2},
  pages={655--668},
  year={2017},
  publisher={IEEE}
}

@article{o2018over,
  title={Over-the-air deep learning based radio signal classification},
  author={O’Shea, Timothy James and Roy, Tamoghna and Clancy, T Charles},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={12},
  number={1},
  pages={168--179},
  year={2018},
  publisher={IEEE}
}

@inproceedings{oyedare2019estimating,
  title={Estimating the Required Training Dataset Size for Transmitter Classification Using Deep Learning},
  author={Oyedare, Taiwo and Park, Jung-Min Jerry},
  booktitle={2019 IEEE International Symposium on Dynamic Spectrum Access Networks (DySPAN)},
  pages={1--10},
  year={2019},
  organization={IEEE}
}

@inproceedings{shi2019deep,
  title={Deep Learning for RF Signal Classification in Unknown and Dynamic Spectrum Environments},
  author={Shi, Yi and Davaslioglu, Kemal and Sagduyu, Yalin E and Headley, William C and Fowler, Michael and Green, Gilbert},
  booktitle={2019 IEEE International Symposium on Dynamic Spectrum Access Networks (DySPAN)},
  pages={1--10},
  year={2019},
  organization={IEEE}
}

@inproceedings{sankhe2019oracle,
  title={ORACLE: Optimized Radio clAssification through Convolutional neuraL nEtworks},
  author={Sankhe, Kunal and Belgiovine, Mauro and Zhou, Fan and Riyaz, Shamnaz and Ioannidis, Stratis and Chowdhury, Kaushik},
  booktitle={IEEE INFOCOM 2019-IEEE Conference on Computer Communications},
  pages={370--378},
  year={2019},
  organization={IEEE}
}

@article{xie2019deep,
  title={Deep learning in digital modulation recognition using high order cumulants},
  author={Xie, Wenwu and Hu, Sheng and Yu, Chao and Zhu, Peng and Peng, Xin and Ouyang, Jingcheng},
  journal={IEEE Access},
  volume={7},
  pages={63760--63766},
  year={2019},
  publisher={IEEE}
}

@misc{polikar1996wavelet,
  title={The wavelet tutorial},
  author={Polikar, Robi and others},
  year={1996}
}

@article{merchant2018deep,
  title={Deep learning for {RF} device fingerprinting in cognitive communication networks},
  author={Merchant, Kevin and Revay, Shauna and Stantchev, George and Nousain, Bryan},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={12},
  number={1},
  pages={160--167},
  year={2018},
  publisher={IEEE}
}

@article{zhou2019robust,
  title={A robust modulation classification method using convolutional neural networks},
  author={Zhou, Siyang and Yin, Zhendong and Wu, Zhilu and Chen, Yunfei and Zhao, Nan and Yang, Zhutian},
  journal={EURASIP Journal on Advances in Signal Processing},
  volume={2019},
  number={1},
  pages={21},
  year={2019},
  publisher={Springer}
}

@inproceedings{davaslioglu2018generative,
  title={Generative adversarial learning for spectrum sensing},
  author={Davaslioglu, Kemal and Sagduyu, Yalin E},
  booktitle={2018 IEEE International Conference on Communications (ICC)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}

@article{riyaz2018deep,
  title={Deep learning convolutional neural networks for radio identification},
  author={Riyaz, Shamnaz and Sankhe, Kunal and Ioannidis, Stratis and Chowdhury, Kaushik},
  journal={IEEE Communications Magazine},
  volume={56},
  number={9},
  pages={146--152},
  year={2018},
  publisher={IEEE}
}

@inproceedings{karra2017modulation,
  title={Modulation recognition using hierarchical deep neural networks},
  author={Karra, Krishna and Kuzdeba, Scott and Petersen, Josh},
  booktitle={2017 IEEE International Symposium on Dynamic Spectrum Access Networks (DySPAN)},
  pages={1--3},
  year={2017},
  organization={IEEE}
}


@article{tang2018digital,
  title={Digital signal modulation classification with data augmentation using generative adversarial nets in cognitive radio networks},
  author={Tang, Bin and Tu, Ya and Zhang, Zhaoyue and Lin, Yun},
  journal={IEEE Access},
  volume={6},
  pages={15713--15722},
  year={2018},
  publisher={IEEE}
}

@inproceedings{mun2020automotive,
  title={Automotive radar signal interference mitigation using {RNN} with self attention},
  author={Mun, Jiwoo and Ha, Seokhyeon and Lee, Jungwoo},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3802--3806},
  year={2020},
  organization={IEEE}
}

@article{rock2021resource,
  title={Resource-Efficient Deep Neural Networks for Automotive Radar Interference Mitigation},
  author={Rock, Johanna and Roth, Wolfgang and Toth, Mate and Meissner, Paul and Pernkopf, Franz},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={15},
  number={4},
  pages={927--940},
  year={2021},
  publisher={IEEE}
}

@misc{hubens_2018, title={Deep inside: Autoencoders}, url={https://towardsdatascience.com/deep-inside-autoencoders-7e41f319999f}, journal={Towards Data Science}, publisher={Medium}, author={Hubens, Nathan}, year={2018}, month={Feb}}

@inproceedings{chen2021dnn,
  title={A {DNN} Autoencoder for Automotive Radar Interference Mitigation},
  author={Chen, Shengyi and Taghia, Jalal and Fei, Tai and K{\"u}hnau, Uwe and Pohl, Nils and Martin, Rainer},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={4065--4069},
  year={2021},
  organization={IEEE}
}

@misc{jordan_2018, title={Introduction to Autoencoders}, url={https://www.jeremyjordan.me/autoencoders/}, journal={Data Science}, author={Jordan, Jeremy}, year={2018}, month={Mar}}

@article{morawski2021anomaly,
  title={Anomaly Detection in Gravitational Waves data using Convolutional AutoEncoders},
  author={Morawski, Filip and Bejger, Micha{\l} Stanis{\l}aw and Cuoco, Elena and Petre, Luigia},
  journal={Machine Learning: Science and Technology},
  year={2021},
  publisher={IOP Publishing}
}

@inproceedings{fuchs2021complex,
  title={Complex-valued Convolutional Neural Networks for Enhanced Radar Signal Denoising and Interference Mitigation},
  author={Fuchs, Alexander and Rock, Johanna and Toth, Mate and Meissner, Paul and Pernkopf, Franz},
  booktitle={2021 IEEE Radar Conference (RadarConf21)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@inproceedings{hager2018nonlinear,
  title={Nonlinear interference mitigation via deep neural networks},
  author={H{\"a}ger, Christian and Pfister, Henry D},
  booktitle={2018 Optical Fiber Communications Conference and Exposition (OFC)},
  pages={1--3},
  year={2018},
  organization={IEEE}
}

@article{wei2016gps,
  title={{GPS} interference mitigation using derivative-free kalman filter-based {RNN}},
  author={Wei-Lung, M},
  journal={Radioengineering},
  volume={25},
  number={3},
  pages={519},
  year={2016}
}

@inproceedings{promsuk2021development,
  title={Development of Interference Mitigation Techniques based Artificial Neural Network for {IoT} Network},
  author={Promsuk, Natthanan},
  booktitle={2021 18th International Conference on Electrical Engineering/Electronics, Computer, Telecommunications and Information Technology (ECTI-CON)},
  pages={374--377},
  year={2021},
  organization={IEEE}
}

@article{kulin2018end,
  title={End-to-end learning from spectrum data: A deep learning approach for wireless signal identification in spectrum monitoring applications},
  author={Kulin, Merima and Kazaz, Tarik and Moerman, Ingrid and De Poorter, Eli},
  journal={IEEE Access},
  volume={6},
  pages={18484--18501},
  year={2018},
  publisher={IEEE}
}

@article{mosavi2016narrowband,
  title={Narrowband interference suppression for {GPS} navigation using neural networks},
  author={Mosavi, MR and Shafiee, F},
  journal={GPS solutions},
  volume={20},
  number={3},
  pages={341--351},
  year={2016},
  publisher={Springer}
}

@inproceedings{shi2012interference,
  title={Interference Suppression for Satellite Navigation Based on Neural Network and Wavelet Packets Transform},
  author={Shi, Yang Chun and Liu, You Bao},
  booktitle={Advanced Materials Research},
  volume={457},
  pages={1111--1117},
  year={2012},
  organization={Trans Tech Publ}
}

@article{liu2021detecting,
  title={Detecting Out-of-Distribution Data in Wireless Communications Applications of Deep Learning},
  author={Liu, Jinshan and Oyedare, Taiwo and Park, Jung-Min},
  journal={IEEE Transactions on Wireless Communications},
  year={2021},
  publisher={IEEE}
}

@article{chung2014empirical,
  title={Empirical evaluation of gated recurrent neural networks on sequence modeling},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, KyungHyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1412.3555},
  year={2014}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  pages={5998--6008},
  year={2017}
}

@article{connor1994recurrent,
  title={Recurrent neural networks and robust time series prediction},
  author={Connor, Jerome T and Martin, R Douglas and Atlas, Les E},
  journal={{IEEE} transactions on neural networks},
  volume={5},
  number={2},
  pages={240--254},
  year={1994},
  publisher={IEEE}
}

@article{torrence1998practical,
  title={A practical guide to wavelet analysis},
  author={Torrence, Christopher and Compo, Gilbert P},
  journal={Bulletin of the American Meteorological society},
  volume={79},
  number={1},
  pages={61--78},
  year={1998},
  publisher={American Meteorological Society}
}


@inproceedings{mattei2019feature,
  title={Feature Learning for Enhanced Security in the Internet of Things},
  author={Mattei, Enrico and Dalton, Cass and Draganov, Andrew and Marin, Brent and Tinston, Michael and Harrison, Greg and Smarrelli, Bob and Harlacher, Marc},
  booktitle={2019 {IEEE} Global Conference on Signal and Information Processing (GlobalSIP)},
  pages={1--5},
  year={2019},
  organization={IEEE}
}


@inproceedings{morin2019transmitter,
  title={Transmitter classification with supervised deep learning},
  author={Morin, Cyrille and Cardoso, Leonardo S and Hoydis, Jakob and Gorce, Jean-Marie and Vial, Thibaud},
  booktitle={International Conference on Cognitive Radio Oriented Wireless Networks},
  pages={73--86},
  year={2019},
  organization={Springer}
}


@article{lee2017deep,
  title={Deep sensing: Cooperative spectrum sensing based on convolutional neural networks},
  author={Lee, Woongsup and Kim, Minhoe and Cho, Dong-Ho},
  journal={arXiv preprint arXiv:1705.08164},
  year={2017}
}


@misc{matlab,
  title = {{CWT}-Based Time-Frequency Analysis},
  howpublished = {https://www.mathworks.com/help/wavelet/examples/cwt-based-time-frequency-analysis.html},
  note = {Accessed: 2019-06-6}
}

@misc{ristea2020dataset,
  title = {Automotive Radar Interference Mitigation data sets ({ARIM})},
  howpublished = {https://github.com/ristea/arim},
  note = {Accessed: 2021-12-08}
}

@inproceedings{xu2020open,
  title={Open-Set Interference Signal Recognition Using Boundary Samples: A Hybrid Approach},
  author={Xu, Yujie and Qin, Xiaowei and Xu, Xiaodong and Chen, Jianqiang},
  booktitle={2020 International Conference on Wireless Communications and Signal Processing (WCSP)},
  pages={269--274},
  year={2020},
  organization={IEEE}
}

@article{palicot2003new,
  title={A new concept for wireless reconfigurable receivers},
  author={Palicot, Jacques and Roland, Christian},
  journal={IEEE Communications Magazine},
  volume={41},
  number={7},
  pages={124--132},
  year={2003},
  publisher={IEEE}
}

@article{courtat2020light,
  title={A light neural network for modulation detection under impairments},
  author={Courtat, Thomas and Bourboux, H{\'e}lion du Mas des},
  journal={arXiv preprint arXiv:2003.12260},
  year={2020}
}

@inproceedings{kim2018identifying,
  title={Identifying signal source using channel state information in wireless {LANs}},
  author={Kim, Yonghwi and An, Sanghyun and So, Jungmin},
  booktitle={2018 International Conference on Information Networking (ICOIN)},
  pages={616--621},
  year={2018},
  organization={IEEE}
}

@inproceedings{draganov2020open,
  title={Open set recognition through unsupervised and class-distance learning},
  author={Draganov, Andrew and Brown, Carter and Mattei, Enrico and Dalton, Cass and Ranjit, Jaspreet},
  booktitle={Proceedings of the 2nd ACM Workshop on Wireless Security and Machine Learning},
  pages={7--12},
  year={2020}
}

@article{peng2018modulation,
  title={Modulation classification based on signal constellation diagrams and deep learning},
  author={Peng, Shengliang and Jiang, Hanyu and Wang, Huaxia and Alwageed, Hathal and Zhou, Yu and Sebdani, Marjan Mazrouei and Yao, Yu-Dong},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={30},
  number={3},
  pages={718--727},
  year={2018},
  publisher={IEEE}
}


%%%%%%%%%%%%%%%% VAE References

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@article{kingma2014semi,
  title={Semi-supervised learning with deep generative models},
  author={Kingma, Diederik P and Rezende, Danilo J and Mohamed, Shakir and Welling, Max},
  journal={arXiv preprint arXiv:1406.5298},
  year={2014}
}

@article{an2015variational,
  title={Variational autoencoder based anomaly detection using reconstruction probability},
  author={An, Jinwon and Cho, Sungzoon},
  journal={Special Lecture on IE},
  volume={2},
  number={1},
  pages={1--18},
  year={2015}
}

@article{higgins2016beta,
  title={$\beta$-vae: Learning basic visual concepts with a constrained variational framework},
  author={Higgins, Irina and Matthey, Loic and Pal, Arka and Burgess, Christopher and Glorot, Xavier and Botvinick, Matthew and Mohamed, Shakir and Lerchner, Alexander},
  year={2016}
}

@article{dilokthanakul2016deep,
  title={Deep unsupervised clustering with gaussian mixture variational autoencoders},
  author={Dilokthanakul, Nat and Mediano, Pedro AM and Garnelo, Marta and Lee, Matthew CH and Salimbeni, Hugh and Arulkumaran, Kai and Shanahan, Murray},
  journal={arXiv preprint arXiv:1611.02648},
  year={2016}
}


@inproceedings{theis2016note,
  title={A note on the evaluation of generative models},
  author={Theis, L and van den Oord, A and Bethge, M},
  booktitle={International Conference on Learning Representations (ICLR 2016)},
  pages={1--10},
  year={2016}
}

@article{burgess2018understanding,
  title={Understanding disentangling in $\beta$-VAE},
  author={Burgess, Christopher P and Higgins, Irina and Pal, Arka and Matthey, Loic and Watters, Nick and Desjardins, Guillaume and Lerchner, Alexander},
  journal={arXiv preprint arXiv:1804.03599},
  year={2018}
}


@inproceedings{kingma2018glow,
  title={Glow: Generative flow with invertible 1x1 convolutions},
  author={Kingma, Durk P and Dhariwal, Prafulla},
  booktitle={Advances in Neural Information Processing Systems},
  pages={10215--10224},
  year={2018}
}


@inproceedings{xu2018unsupervised,
  title={Unsupervised anomaly detection via variational auto-encoder for seasonal kpis in web applications},
  author={Xu, Haowen and Chen, Wenxiao and Zhao, Nengwen and Li, Zeyan and Bu, Jiahao and Li, Zhihan and Liu, Ying and Zhao, Youjian and Pei, Dan and Feng, Yang and others},
  booktitle={Proceedings of the 2018 World Wide Web Conference},
  pages={187--196},
  year={2018}
}

@article{klushyn2019learning,
  title={Learning hierarchical priors in VAEs},
  author={Klushyn, Alexej and Chen, Nutan and Kurle, Richard and Cseke, Botond and van der Smagt, Patrick},
  journal={arXiv preprint arXiv:1905.04982},
  year={2019}
}

@article{daxberger2019bayesian,
  title={Bayesian variational autoencoders for unsupervised out-of-distribution detection},
  author={Daxberger, Erik and Hern{\'a}ndez-Lobato, Jos{\'e} Miguel},
  journal={arXiv preprint arXiv:1912.05651},
  year={2019}
}

@article{zhang2020out,
  title={Out-of-Distribution Detection with Distance Guarantee in Deep Generative Models},
  author={Zhang, Yufeng and Liu, Wanwei and Chen, Zhenbang and Wang, Ji and Liu, Zhiming and Li, Kenli and Wei, Hongmei and Chen, Zuoning},
  journal={arXiv preprint arXiv:2002.03328},
  year={2020}
}

%%%%%%%%%%%%%%%% OOD References

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}


@inproceedings{nguyen2015deep,
  title={Deep neural networks are easily fooled: High confidence predictions for unrecognizable images},
  author={Nguyen, Anh and Yosinski, Jason and Clune, Jeff},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={427--436},
  year={2015}
}


@article{hendrycks2016baseline,
  title={A baseline for detecting misclassified and out-of-distribution examples in neural networks},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1610.02136},
  year={2016}
}

@inproceedings{liang2018enhancing,
  title={Enhancing The Reliability of Out-of-distribution Image Detection in Neural Networks},
  author={Liang, Shiyu and Li, Yixuan and Srikant, R},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{lakshminarayanan2017simple,
  title={Simple and scalable predictive uncertainty estimation using deep ensembles},
  author={Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6402--6413},
  year={2017}
}

@inproceedings{lee2018training,
  title={Training Confidence-calibrated Classifiers for Detecting Out-of-Distribution Samples},
  author={Lee, Kimin and Lee, Honglak and Lee, Kibok and Shin, Jinwoo},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{moosavi2017universal,
  title={Universal adversarial perturbations},
  author={Moosavi-Dezfooli, Seyed-Mohsen and Fawzi, Alhussein and Fawzi, Omar and Frossard, Pascal},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1765--1773},
  year={2017}
}

@inproceedings{hendrycks2018deep,
  title={Deep Anomaly Detection with Outlier Exposure},
  author={Hendrycks, Dan and Mazeika, Mantas and Dietterich, Thomas},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{malinin2018predictive,
  title={Predictive uncertainty estimation via prior networks},
  author={Malinin, Andrey and Gales, Mark},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7047--7058},
  year={2018}
}

@inproceedings{kendall2018multi,
  title={Multi-task learning using uncertainty to weigh losses for scene geometry and semantics},
  author={Kendall, Alex and Gal, Yarin and Cipolla, Roberto},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7482--7491},
  year={2018}
}

@inproceedings{kendall2017uncertainties,
  title={What uncertainties do we need in bayesian deep learning for computer vision?},
  author={Kendall, Alex and Gal, Yarin},
  booktitle={Advances in neural information processing systems},
  pages={5574--5584},
  year={2017}
}


@inproceedings{vyas2018out,
  title={Out-of-distribution detection using an ensemble of self supervised leave-out classifiers},
  author={Vyas, Apoorv and Jammalamadaka, Nataraj and Zhu, Xia and Das, Dipankar and Kaul, Bharat and Willke, Theodore L},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={550--564},
  year={2018}
}

@inproceedings{nalisnick2018deep,
  title={Do Deep Generative Models Know What They Don't Know?},
  author={Nalisnick, Eric and Matsukawa, Akihiro and Teh, Yee Whye and Gorur, Dilan and Lakshminarayanan, Balaji},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@article{choi2018waic,
  title={Waic, but why? generative ensembles for robust anomaly detection},
  author={Choi, Hyunsun and Jang, Eric and Alemi, Alexander A},
  journal={arXiv preprint arXiv:1810.01392},
  year={2018}
}

@inproceedings{lee2018simple,
  title={A simple unified framework for detecting out-of-distribution samples and adversarial attacks},
  author={Lee, Kimin and Lee, Kibok and Lee, Honglak and Shin, Jinwoo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7167--7177},
  year={2018}
}

@inproceedings{ren2019likelihood,
  title={Likelihood ratios for out-of-distribution detection},
  author={Ren, Jie and Liu, Peter J and Fertig, Emily and Snoek, Jasper and Poplin, Ryan and Depristo, Mark and Dillon, Joshua and Lakshminarayanan, Balaji},
  booktitle={Advances in Neural Information Processing Systems},
  pages={14680--14691},
  year={2019}
}


@article{nalisnick2019detecting,
  title={Detecting out-of-distribution inputs to deep generative models using a test for typicality},
  author={Nalisnick, Eric and Matsukawa, Akihiro and Teh, Yee Whye and Lakshminarayanan, Balaji},
  journal={arXiv preprint arXiv:1906.02994},
  year={2019}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={IEEE}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{ioffe2015batch,
  title={Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  booktitle={International Conference on Machine Learning},
  pages={448--456},
  year={2015}
}

@article{radford2015unsupervised,
  title={Unsupervised representation learning with deep convolutional generative adversarial networks},
  author={Radford, Alec and Metz, Luke and Chintala, Soumith},
  journal={arXiv preprint arXiv:1511.06434},
  year={2015}
}


@inproceedings{chen2016infogan,
  title={Infogan: Interpretable representation learning by information maximizing generative adversarial nets},
  author={Chen, Xi and Duan, Yan and Houthooft, Rein and Schulman, John and Sutskever, Ilya and Abbeel, Pieter},
  booktitle={Advances in neural information processing systems},
  pages={2172--2180},
  year={2016}
}

@article{youssef2018machine,
  title={Machine learning approach to {RF} transmitter identification},
  author={Youssef, Khalid and Bouchard, Louis and Haigh, Karen and Silovsky, Jan and Thapa, Bishal and Vander Valk, Chris},
  journal={IEEE Journal of Radio Frequency Identification},
  volume={2},
  number={4},
  pages={197--205},
  year={2018},
  publisher={IEEE}
}
